Joint Superposition Coding and Training for Federated Learning over Multi-Width Neural Networks

This paper aims to integrate two synergetic technologies, federated learning (FL) and width-adjustable slimmable neural network (SNN) architectures. FL preserves data privacy by exchanging the locally trained models of mobile devices. By adopting SNNs as local models, FL can flexibly cope with the time-varying energy capacities of mobile devices. Combining FL and SNNs is however non-trivial, particularly under wireless connections with time-varying channel conditions. Furthermore, existing multi-width SNN training algorithms are sensitive to the data distributions across devices, so are ill-suited to FL. Motivated by this, we propose a communication and energy-efficient SNN-based FL (named SlimFL) that jointly utilizes superposition coding (SC) for global model aggregation and superposition training (ST) for updating local models. By applying SC, SlimFL exchanges the superposition of multiple width configurations that are decoded as many as possible for a given communication throughput. Leveraging ST, SlimFL aligns the forward propagation of different width configurations, while avoiding the inter-width interference during backpropagation. We formally prove the convergence of SlimFL. The result reveals that SlimFL is not only communication-efficient but also can counteract non-IID data distributions and poor channel conditions, which is also corroborated by simulations.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
% \def\eqref#1{eqn.~(\ref{#1})}
% Reference to an equation, upper case
% \def\Eqref#1{Eqn.~\ref{#1}}
% A raw reference to an equation---avoid using if possible
% \def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\def\A{{\bf A}}
\def\a{{\bf a}}
\def\B{{\bf B}}
\def\bb{{\bf b}}
\def\C{{\bf C}}
\def\c{{\bf c}}
\def\D{{\bf D}}
\def\d{{\bf d}}
\def\E{{\bf E}}
\def\e{{\bf e}}
\def\F{{\bf F}}
\def\f{{\bf f}}
\def\g{{\bf g}}
\def\h{{\bf h}}
\def\G{{\bf G}}
\def\H{{\bf H}}
\def\I{{\bf I}}
\def\K{{\bf K}}
\def\k{{\bf k}}
\def\LL{{\bf L}}
\def\l{{\bf l}}
\def\M{{\bf M}}
\def\m{{\bf m}}
\def\N{{\bf N}}
\def\n{{\bf n}}
\def\oo{{\bf o}}
\def\PP{{\bf P}}
\def\Q{{\bf Q}}
\def\q{{\bf q}}
\def\R{{\bf R}}
\def\rr{{\bf r}}
\def\S{{\bf S}}
\def\s{{\bf s}}
\def\T{{\bf T}}
\def\tt{{\bf t}}
\def\U{{\bf U}}
\def\u{{\bf u}}
\def\V{{\bf V}}
\def\v{{\bf v}}
\def\W{{\bf W}}
\def\w{{\bf w}}
\def\X{{\bf X}}
\def\x{{\bf x}}
\def\Y{{\bf Y}}
\def\y{{\bf y}}
\def\Z{{\bf Z}}
\def\z{{\bf z}}
\def\0{{\bf 0}}
\def\1{{\bf 1}}

\def\AM{{\mathcal A}}
\def\CM{{\mathcal C}}
\def\DM{{\mathcal D}}
\def\EM{{\mathcal E}}
\def\GM{{\mathcal G}}
\def\FM{{\mathcal F}}
\def\IM{{\mathcal I}}
\def\HM{{\mathcal H}}
\def\JM{{\mathcal J}}
\def\KM{{\mathcal K}}
\def\LM{{\mathcal L}}
\def\NM{{\mathcal N}}
\def\OM{{\mathcal O}}
\def\PM{{\mathcal P}}
\def\SM{{\mathcal S}}
\def\TM{{\mathcal T}}
\def\UM{{\mathcal U}}
\def\VM{{\mathcal V}}
\def\WM{{\mathcal W}}
\def\XM{{\mathcal X}}
\def\YM{{\mathcal Y}}
\def\ZM{{\mathcal Z}}
\def\CB{{\mathbb C}}
\def\RB{{\mathbb R}}
\def\EB{{\mathbb E}}
\def\ZB{{\mathbb Z}}
\def\PB{{\mathbb P}}
\def\OB{{\mathbb O}}

\def\alp{\mbox{\boldmath$\alpha$\unboldmath}}
\def\bet{\mbox{\boldmath$\beta$\unboldmath}}
\def\epsi{\mbox{\boldmath$\epsilon$\unboldmath}}
\def\varepsi{\mbox{\boldmath$\varepsilon$\unboldmath}}
\def\etab{\mbox{\boldmath$\eta$\unboldmath}}
\def\pii{\mbox{\boldmath$\pi$\unboldmath}}
\def\Ph{\mbox{\boldmath$\Phi$\unboldmath}}
\def\ph{\mbox{\boldmath$\phi$\unboldmath}}
\def\Ps{\mbox{\boldmath$\Psi$\unboldmath}}
\def\ps{\mbox{\boldmath$\psi$\unboldmath}}
\def\tha{\mbox{\boldmath$\theta$\unboldmath}}
\def\Tha{\mbox{\boldmath$\Theta$\unboldmath}}
\def\muu{\mbox{\boldmath$\mu$\unboldmath}}
\def\Si{\mbox{\boldmath$\Sigma$\unboldmath}}
\def\si{\mbox{\boldmath$\sigma$\unboldmath}}
\def\Gam{\mbox{\boldmath$\Gamma$\unboldmath}}
\def\Lam{\mbox{\boldmath$\Lambda$\unboldmath}}
\def\lam{\mbox{\boldmath$\lambda$\unboldmath}}
\def\De{\mbox{\boldmath$\Delta$\unboldmath}}
\def\Ome{\mbox{\boldmath$\Omega$\unboldmath}}
\def\Pii{\mbox{\boldmath$\Pi$\unboldmath}}
\def\Xii{\mbox{\boldmath$\Xi$\unboldmath}}
\def\xii{\mbox{\boldmath$\xi$\unboldmath}}
\def\vps{\mbox{\boldmath$\varepsilon$\unboldmath}}
\def\argmax{\mathop{\rm argmax}}
\def\argmin{\mathop{\rm argmin}}

\def\sumk{\sum_{k \in \mathcal{S}_t}}
\def\bias{\mathsf{bias}}
\def\var{\mathsf{var}}
\def\nnz{\mathrm{nnz}}
\def\poly{\mathrm{poly}}
\def\cov{\mathrm{cov}}
\def\sgn{\mathrm{sgn}}
\def\range{\mathrm{range}}
\def\nul{\mathrm{null}}
\def\tr{\mathrm{tr}}
\def\rk{\mathrm{rank}}
\def\diag{\mathrm{diag}}
\def\const{\mathrm{Const}}
\def\dg{\mathsf{dg}}
\def\st{\mathsf{s.t.}}
\def\vect{\mathsf{vec}}
\def\etal{{\em et al.\/}\,}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

%\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
%\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


\newcommand{\aw}{\overline{\w}}
\newcommand{\avg}{\overline{\vg}}
\newcommand{\IB}[1]{\mathbb{I}\left\{#1\right\}}
% \newcommand{\myave}{\mathrm{ave}}
\newcommand{\myave}{\sum_{k=1}^N}
\newcommand{\ESt}{\EB_{\SM_t}}
\newcommand{\av}{\overline{\v}}

==> tex/convergence_proof.tex <==

\section{Proof of Theorem~\ref{thm:full}}
\label{appen:full}
We analyze \texttt{FedAvg} in the setting of full device participation in this section.

\subsection{Additional Notation}
Let $\w_t^k$ be the model parameter maintained in the $k$-th device at the $t$-th step. Let $\IM_E$ be the set of global synchronization steps, i.e., $\IM_E = \{nE \  | \ n=1,2,\cdots\}$. If $t+1 \in \IM_E$, i.e., the time step to communication, \texttt{FedAvg} activates all devices. Then the update of \texttt{FedAvg} with partial devices active can be described as
\begin{align}
& \v_{t+1}^k = \w_t^k - \eta_t \nabla F_k(\w_t^k, \xi_t^k), 
\label{eq:update_pre}\\
& \w_{t+1}^k =\left\{\begin{array}{ll}
\v_{t+1}^k           & \text{ if } t+1 \notin \IM_E, \\
\sum_{k=1}^N p_k \v_{t+1}^k   & \text{ if } t+1  \in \IM_E.
\label{eq:ave_pre}
\end{array}\right. 
\end{align}
Here, an additional variable $\v_{t+1}^k$ is introduced to represent the immediate result of one step SGD update from $\w_t^k$. We interpret $\w_{t+1}^k$ as the parameter obtained after communication steps (if possible).

In our analysis, we define two virtual sequences $\av_t = \myave \v_t^k$ and $\aw_t = \myave \w_t^k$. This is motivated by \citep{stich2018local}. $\av_{t+1}$ results from an single step of SGD from $\aw_{t}$. 
When $t+1 \notin \IM_E$, both are inaccessible. When $t+1 \in \IM_E$, we can only fetch $\aw_{t+1}$. For convenience, we define $\overline{\g}_t = \myave \nabla F_k(\w_t^k)$ and $\g_t = \myave \nabla F_k(\w_t^k, \xi_t^k)$.  
Therefore, $\overline{\v}_{t+1} = \overline{\w}_t - \eta_t \g_t$ and $\EB \g_t = \overline{\g}_t$.


\subsection{Key Lemmas}
To convey our proof clearly, it would be necessary to prove certain useful lemmas. We defer the proof of these lemmas to latter section and focus on proving the main theorem.

\begin{lem}[Results of one step SGD]
\label{lem:conv_main} Assume Assumption~\ref{asm:smooth} and~\ref{asm:strong_cvx}. If $\eta_t\leq \frac{1}{4L}$, we have
\[  
\EB \left\|\overline{\v}_{t+1}-\w^{\star}\right\|^{2} 
\leq (1-\eta_t \mu) \EB \left\|\overline{\w}_{t}-\w^{\star}\right\|^{2} 
+ \eta_{t}^{2} \EB \left\|\mathbf{g}_{t}-\overline{\mathbf{g}}_{t}\right\|^{2} + 6L \eta_t^2 \Gamma 
+ 2 \EB \myave \left\|\overline{\w}_{t}-\w_{k}^{t}\right\|^{2} 
\]
where $\Gamma = F^* - \myave F_k^{\star} \ge 0$.
\end{lem}


\begin{lem}[Bounding the variance]
Assume Assumption~\ref{asm:sgd_var} holds. It follows that
	\label{lem:conv_variance}
	\[\EB \left\|\mathbf{g}_{t}-\overline{\mathbf{g}}_{t}\right\|^{2}  \leq \sum_{k=1}^N p_k^2 \sigma_k^2.\]
\end{lem}


\begin{lem}[Bounding the divergence of $\{\w_t^k\}$]
	\label{lem:conv_diversity}
	Assume Assumption~\ref{asm:sgd_norm}, that $\eta_t$ is non-increasing and $\eta_{t} \le 2 \eta_{t+E}$ for all $t\geq 0$. It follows that
	\[\EB \left[ \myave \left\|\overline{\w}_{t}-\w_{k}^{t}\right\|^{2} \right]
	\: \leq \: 4 \eta_t^2 (E-1)^2 G^2.\]
\end{lem}

\subsection{Completing the Proof of Theorem~\ref{thm:full}}
\begin{proof}
It is clear that no matter whether $t+1 \in \IM_E$ or $t+1 \notin \IM_E$, we always have $\aw_{t+1}= \av_{t+1}$. Let $\Delta_t=\EB \left\|\aw_{t}-\w^{\star}\right\|^{2}$. From Lemma~\ref{lem:conv_main}, Lemma~\ref{lem:conv_variance} and Lemma~\ref{lem:conv_diversity}, it follows that
\begin{equation}
\label{eq:conv_full_final}
\Delta_{t+1} \le (1-\eta_t \mu) \Delta_t + \eta_t^2 B
\end{equation}
where
\[ B = \sum_{k=1}^N p_k^2 \sigma_k^2 +  6L \Gamma + 8 (E-1)^2G^2. \]

 For a diminishing stepsize, $\eta_t = \frac{\beta}{t + \gamma}$ for some $\beta > \frac{1}{\mu}$ and $\gamma > 0$ such that $\eta_1 \le \min\{\frac{1}{\mu}, \frac{1}{4L}\}=\frac{1}{4L}$ and $\eta_{t} \le 2 \eta_{t+E}$. We will prove $\Delta_t \le \frac{v}{\gamma + t}$ where $v = \max\left\{ \frac{\beta^2 B}{\beta \mu -1}, (\gamma+1)\Delta_1 \right\}$.

We prove it by induction. Firstly, the definition of $v$ ensures that it holds for $t = 1$. Assume the conclusion holds for some $t$, it follows that
\begin{align*}
\Delta_{t+1} 
&\le (1-\eta_t\mu )\Delta_t + \eta_t^2 B \\
&\le \left(1- \frac{\beta\mu}{t + \gamma}\right)\frac{v}{t + \gamma} + \frac{\beta^2B}{(t + \gamma)^2}\\
&=\frac{t + \gamma -1}{(t + \gamma)^2} v  + \left[ \frac{\beta^2B}{(t + \gamma)^2} - \frac{\beta\mu-1}{(t+\gamma)^2}v \right] \\
& \le \frac{v}{t + \gamma +1}.
\end{align*}

Then by the $L$-smoothness of $F(\cdot)$,
\[  \EB [F(\aw_t)] - F^* \le \frac{L}{2} \Delta_t  \le \frac{L}{2} \frac{v}{\gamma + t}.\]
Specifically, if we choose $\beta = \frac{2}{\mu}, \gamma = \max\{8 \frac{L}{\mu}, E\}-1$ and denote $\kappa = \frac{L}{\mu}$, then  $\eta_t = \frac{2}{\mu} \frac{1}{\gamma + t}$.
One can verify that the choice of $\eta_{t}$ satisfies $\eta_{t} \le 2\eta_{t+E}$ for $t \ge 1$.
Then, we have
\[
v = \max\left\{ \frac{\beta^2 B}{\beta \mu -1}, (\gamma+1)\Delta_1 \right\} 
\le \frac{\beta^2 B}{\beta \mu -1} +  (\gamma+1)\Delta_1 \le 
\frac{4B}{\mu^2} + (\gamma+1) \Delta_1,
\]
and 
\[  \EB [F(\aw_t)] - F^*
 \le   \frac{L}{2} \frac{v}{\gamma + t} 
 \le   \frac{\kappa}{\gamma + t} \left( \frac{2B}{\mu} +   \frac{\mu (\gamma+1)}{2} \Delta_1 \right). \]
\end{proof}


\subsection{Deferred proofs of key lemmas}
\begin{proof}[Proof of Lemma~\ref{lem:conv_main}.]
	Notice that $\av_{t+1} = \aw_t - \eta_t \vg_t$, then
	\begin{align}
	\label{eq:partial_main}
	\left\|\overline{\v}_{t+1}-\w^{\star}\right\|^{2} \nonumber 
	&=\left\|\overline{\w}_{t}-\eta_{t} \mathbf{g}_{t}-\w^{\star}-\eta_{t} \overline{\mathbf{g}}_{t}+\eta_{t} \overline{\mathbf{g}}_{t}\right\|^{2} \nonumber \\ 
	&=\underbrace{\left\|\overline{\w}_{t}-\w^{\star}-\eta_{t} \overline{\mathbf{g}}_{t}\right\|^{2}}_{A_1}+
	\underbrace{2\eta_{t}\left\langle\overline{\w}_{t}-\w^{\star}-\eta_{t} \overline{\mathbf{g}}_{t}, \overline{\mathbf{g}}_{t}-\mathbf{g}_{t}\right\rangle}_{A_2} +
	\eta_{t}^{2}\left\|\mathbf{g}_{t}-\overline{\mathbf{g}}_{t}\right\|^{2}
	\end{align}
	Note that $\EB A_2 = 0$. We next focus on bounding $A_1$. Again we split $A_1$ into three terms:
	\begin{equation}
	\label{eq:partial_proof_main_term}
	\left\|\overline{\w}_{t}-\w^{\star}-\eta_{t} \overline{\mathbf{g}}_{t}\right\|^{2} =\left\|\overline{\w}_{t}-\w^{\star}\right\|^{2}
	\underbrace{-2 \eta_{t}\left\langle\overline{\w}_{t}-\w^{\star}, \overline{\mathbf{g}}_{t}\right\rangle}_{B_1}
	+  \underbrace{\eta_{t}^{2}\left\|\overline{\mathbf{g}}_{t}\right\|^{2}}_{B_2}
	\end{equation}
	
	From the the $L$-smoothness of $F_k(\cdot)$, it follows that
	\begin{equation}
	\label{eq:partial_proof_L}
	  \left\|\nabla F_k\left(\w_{t}^{k}\right)\right\|^{2} \leq 2 L\left(F_k\left(\w_{t}^{k}\right)-F_k^{\star}\right).
	\end{equation}
	
	By the convexity of $\left\| \cdot \right \|^2$ and~\eqref{eq:partial_proof_L}, we have
	\[
	B_2 = \eta_{t}^{2}\left\|\overline{\mathbf{g}}_{t}\right\|^{2} 
	\leq \eta_{t}^{2}\myave \left\|\nabla F_k\left(\w_{t}^{k}\right)\right\|^{2}
	\leq 2L\eta_t^2 \myave \left( F_k(\w_t^k) - F_k^*\right).
	\]
	
	Note that 
	\begin{align}
	\label{eq:partial_B1}
	  B_1 
	  &= -2 \eta_{t}\left\langle\overline{\w}_{t}-\w^{\star}, \overline{\mathbf{g}}_{t}\right\rangle 
	  = -2\eta_t \myave \left\langle\overline{\w}_{t}-\w^{\star}, \nabla F_k(\w_t^k)\right\rangle \nonumber \\
	  &=-2\eta_t \myave \left\langle\overline{\w}_{t}-\w_t^k, \nabla F_k(\w_t^k)\right\rangle
	  -2\eta_t \myave \left\langle\w_t^k-\w^{\star}, \nabla F_k(\w_t^k)\right\rangle.
	\end{align}
	
	By Cauchy-Schwarz inequality and AM-GM inequality, we have
	\begin{equation}
	\label{eq:partial_B11}
	-2 \left\langle\overline{\w}_{t}-\w_t^{k}, \nabla F_k \left(\w_{t}^{k}\right)\right\rangle \leq \frac{1}{\eta_t} \left\|\overline{\w}_{t}-\w_{t}^{k}\right\|^{2}
	+ \eta_t \left\|\nabla F_k\left(\w_{t}^{k}\right)\right\|^{2}.	
	\end{equation}
	
	By the $\mu$-strong convexity of $F_k(\cdot)$, we have
	\begin{equation}
	\label{eq:partial_B12}
	-\left\langle\w_{t}^{k}-\w^{\star}, \nabla F_k\left(\w_{t}^{k}\right)\right\rangle \leq -\left(F_k\left(\w_{t}^{k}\right)-F_k(\w^*)\right)-\frac{\mu}{2}\left\|\w_{t}^{k}-\w^{\star}\right\|^{2}.
	\end{equation}
	
	By combining ~\eqref{eq:partial_proof_main_term},~\eqref{eq:partial_B1},~\eqref{eq:partial_B11} and~\eqref{eq:partial_B12}, it follows that
	\begin{align*}
	 A_1 
	 =  \left\|\overline{\w}_{t}-\w^{\star}-\eta_{t} \overline{\mathbf{g}}_{t}\right\|^{2} 
	 &\leq \left\|\overline{\w}_{t}-\w^{\star}\right\|^{2} 
	 + 2L\eta_t^2 \myave \left( F_k(\w_t^k) - F_k^*\right) \\
	 & \quad +\eta_t \myave \left(\frac{1}{\eta_t} \left\|\overline{\w}_{t}-\w_{k}^{t}\right\|^{2}+\eta_t \left\|\nabla F_k\left(\w_{t}^{k}\right)\right\|^{2}\right)  \\ 
	&  \quad -2\eta_t \myave \left( F_k\left(\w_{t}^{k}\right)-F_k(\w^*) + \frac{\mu}{2}\left\|\w_{t}^{k}-\w^{\star}\right\|^{2} \right) \\
	& = (1-\mu\eta_t)\left\|\overline{\w}_{t}-\w^{\star}\right\|^{2} 
	+ \myave \left\|\overline{\w}_{t}-\w_{k}^{t}\right\|^{2} \\
	& \quad + \underbrace{4L\eta_t^2 \myave \left( F_k(\w_t^k) - F_k^*\right) 
	 - 2\eta_t \myave \left(F_k\left(\w_{t}^{k}\right)-F_k(\w^*)\right)}_{C}
	\end{align*}
	where we use~\eqref{eq:partial_proof_L} again.
	
	
	We next aim to bound $C$. We define $\gamma_t = 2\eta_t(1-2L\eta_t)$. Since $\eta_t \leq \frac{1}{4L}$, $\eta_t \le \gamma_t \leq 2\eta_t$. Then we split $C$ into two terms:
	\begin{align*}
	 C &= - 2\eta_t(1-2L\eta_t) \myave \left( F_k(\w_t^k) - F_k^* \right) 
	 + 2\eta_t \myave \left(F_k(\w^*) - F_k^*\right) \\
	 &=-\gamma_t \myave \left( F_k(\w_t^k) - F^* \right)  
	  + (2\eta_t-\gamma_t)\myave  \left( F^*-F_k^*\right)  \\
	 &=\underbrace{-\gamma_t \myave \left( F_k(\w_t^k) - F^* \right)}_{D}
	 +4L\eta_t^2 \Gamma
	\end{align*}
	where in the last equation, we use the notation $\Gamma = \myave \left( F^*-F_k^*\right)=F^* - \myave F_k^*$.
	
	To bound $D$, we have
	\begin{align*}
	\myave \left( F_k(\w_t^k) - F^*  \right)
	 &=\myave \left( F_k(\w_t^k) - F_k(\overline{\w}_t)  \right) 
	 + \myave \left( F_k(\overline{\w}_t) - F^*  \right)\\
	 & \ge \myave\left\langle \nabla F_k(\overline{\w}_t), \overline{\w}_t^k - \overline{\w}_t \right\rangle
	 + \left( F(\aw_t) - F^* \right) \\
	 & \ge - \frac{1}{2} \myave \left[ \eta_t\left\|  \nabla F_k(\overline{\w}_t) \right\|^2 + \frac{1}{\eta_t}\left\|\w_t^k -\overline{\w}_t\right\|^2 \right]
	 + \left( F(\aw_t) - F^* \right) \\
	 & \ge - \myave \left[ \eta_tL \left(F_k(\overline{\w}_t) -F_k^*   \right)
	 + \frac{1}{2\eta_t}\left\|\w_t^k -\overline{\w}_t\right\|^2 \right]
	 + \left( F(\aw_t) - F^* \right)
	\end{align*}
	where the first inequality results from the convexity of $F_k(\cdot)$, the second inequality from AM-GM inequality and the third inequality from~\eqref{eq:partial_proof_L}.
	
	Therefore 
	\begin{align*}
	  C 
	 &= \gamma_t \myave \left[ \eta_tL \left(F_k(\overline{\w}_t) -F_k^*   \right)
	 + \frac{1}{2\eta_t}\left\|\w_t^k -\overline{\w}_t\right\|^2 \right]
	 - \gamma_t \left( F(\aw_t) - F^* \right) + 4L\eta_t^2 \Gamma\\
	 &= \gamma_t(\eta_t L -1 ) \myave \left(F_k(\aw_t) -F^* \right)
	 + \left( 4L\eta_t^2 + \gamma_t\eta_tL \right) \Gamma + \frac{\gamma_t}{2\eta_t } \myave \left\|\w_t^k -\overline{\w}_t\right\|^2 \\
	 &\le 6L\eta_t^2 \Gamma
     + \myave \left\|\w_t^k -\overline{\w}_t\right\|^2 
	\end{align*}
	where in the last inequality, we use the following facts: (1) $\eta_t L -1 \le - \frac{3}{4} \le 0$ and  $\myave \left(F_k(\aw_t) -F^* \right) = F(\aw_t) - F^*\ge 0$ (2) $\Gamma \ge 0$ and $4L\eta_t^2 + \gamma_t\eta_tL \le 6\eta_t^2L$ and (3) $\frac{\gamma_t}{2\eta_t} \le 1$.
	
	Recalling the expression of $A_1$ and plugging $C$ into it, we have
	\begin{align}
	\label{eq:partial_proof_A1}
	  A_1 
	  &= \left\|\overline{\w}_{t}-\w^{\star}-\eta_{t} \overline{\mathbf{g}}_{t}\right\|^{2} \nonumber\\
      &\le (1-\mu\eta_t)\left\|\overline{\w}_{t}-\w^{\star}\right\|^{2} 
	  + 2 \myave \left\|\overline{\w}_{t}-\w_{k}^{t}\right\|^{2} + 6\eta_t^2L \Gamma 
	\end{align}
	Using~\eqref{eq:partial_proof_A1} and taking expectation on both sides of~\eqref{eq:partial_main}, we erase the randomness from stochastic gradients, we complete the proof.
\end{proof}



\begin{proof}[Proof of Lemma~\ref{lem:conv_variance}]
    From Assumption~\ref{asm:sgd_var}, the variance of the stochastic gradients in device $k$ is bounded by $\sigma_k^2$, then
	\begin{align*}
	\EB \left\|\mathbf{g}_{t}-\overline{\mathbf{g}}_{t}\right\|^{2}  & = \EB \left\| \myave (\nabla F_k(\w_t^k,\xi_t^k) - \nabla F_k(\w_t^k))  \right\|^{2}, \\
	&= \myave^2 \EB \left\|  \nabla F_k(\w_t^k,\xi_t^k) - \nabla F_k(\w_t^k)  \right\|^{2}, \\
	& \leq \sum_{k=1}^N p_k^2 \sigma_k^2.
	\end{align*}
\end{proof}


\begin{proof}[Proof of Lemma~\ref{lem:conv_diversity}]
    Since \texttt{FedAvg} requires a communication each $E$ steps. Therefore, for any $t \ge 0$, there exists a $t_0 \leq t$, such that $t-t_0 \leq E-1$ and $\w_{t_0}^k=\aw_{t_0}$ for all $k=1,2,\cdots,N$. Also, we use the fact that $\eta_t$ is non-increasing and $\eta_{t_0} \leq 2 \eta_t$ for all $t-t_0 \leq E-1$, then
	\begin{align*}
	\EB  \myave \left\|\overline{\w}_{t}-\w_{t}^{k}\right\|^{2} &= \EB  \myave \left\|  (\w_{t}^{k} - \aw_{t_0})  - (\overline{\w}_{t} - \aw_{t_0})   \right\|^{2} \\
	&\leq \EB \myave \left\|  \w_{t}^{k} - \aw_{t_0}  \right\|^{2} \\
	& \leq \myave \EB \sum_{t = t_0}^{t-1}(E-1) \eta_t^2 \left\|  \nabla F_k(\w_t^{k},\xi_t^k)     \right\|^2 \\
	& \leq \myave \sum_{t=t_0} ^{t-1} (E-1) \eta_{t_0}^2 G^2 \\
	& \leq \myave  \eta_{t_0}^2 (E-1)^2 G^2 \\
	& \leq 4 \eta_t^2 (E-1)^2 G^2.
	\end{align*}
	Here in the first inequality, we use $\EB \| X - \EB X \|^2 \le \EB \|X\|^2$ where $X = \w_t^{k} - \overline{\w}_{t_0}$ with probability $p_k$.
	In the second inequality, we use Jensen inequality:
	\[
	\left\|  \w_{t}^{k} - \aw_{t_0}  \right\|^{2} = 
	\left\|  \sum_{t=t_0}^{t-1} \eta_{t}  \nabla F_k(\w_t^{k},\xi_t^k)    \right\|^{2}
	\le (t-t_0) \sum_{t=t_0}^{t-1} \eta_{t}^2 \left\|  \nabla F_k(\w_t^{k},\xi_t^k)   \right\|^2.
	\]
	In the third inequality, we use $\eta_{t} \le \eta_{t_0}$ for $t \ge t_0$ and $\EB \|\nabla F_k(\w_t^{k},\xi_t^k)  \|^2 \le G^2$ for $k=1,2,\cdots N$ and $t \ge 1$.
	In the last inequality, we use $\eta_{t_0} \le 2 \eta_{t_0+E} \le 2 \eta_{t}$ for $t_0 \le t \le t_0 + E$.
\end{proof}



\section{Proofs of Theorems~\ref{thm:w_replace} and~\ref{thm:wo_replace}}
\label{appen:prov}

We analyze \texttt{FedAvg} in the setting of partial device participation in this section.

\subsection{Additional Notation}
Recall that $\w_t^k$ is the model parameter maintained in the $k$-th device at the $t$-th step. $\IM_E = \{nE \  | \ n=1,2,\cdots\}$ is the set of global synchronization steps. Unlike the setting in Appendix~\ref{appen:full}, when it is the time to communicate, i.e., $t+1 \in \IM_E$, the scenario considered here is that \texttt{FedAvg} randomly activates a subset of devices according to some sampling schemes. Again, $\overline{\g}_t = \myave \nabla F_k(\w_t^k)$ and $\g_t = \myave F_k(\w_t^k, \xi_t^k)$.  Therefore, $\overline{\v}_{t+1} = \overline{\w}_t - \eta_t \g_t$ and $\EB \g_t = \overline{\g}_t$.


\paragraph{Multiset selected.} 
All sampling schemes can be divided into two groups, one with replacement and the other without replacement. For those with replacement,  it is possible for a device to be activated several times in a round of communication, even though each activation is independent with the rest. We denote by $\HM_t$ the multiset selected which allows any element to appear more than once. Note that $\HM_t$ is only well defined for $t \in \IM_E$. For convenience, we denote by $\SM_t = \HM_{N(t, E)}$ the most recent set of chosen devices where $N(t, E) = \max\{n| n \le t, n \in \IM_E\}$. 


\paragraph{Updating scheme.}
Limited to realistic scenarios (for communication efficiency and low straggler effect), \text{FedAvg} first samples a random multiset $\SM_t$ of devices and then only perform updates on them. This make the analysis a little bit intricate, since $\SM_t$ varies each $E$ steps. However, we can use a thought trick to circumvent this difficulty. We assume that \texttt{FedAvg} always activates \textbf{all devices} at the beginning of each round and then uses the parameters maintained in only a few sampled devices to produce the next-round parameter. It is clear that this updating scheme is equivalent to the original. Then the update of \texttt{FedAvg} with partial devices active can be described as: for all $k \in [N]$,
\begin{align}
& \v_{t+1}^k = \w_t^k - \eta_t \nabla F_k(\w_t^k, \xi_t^k), 
\label{eq:partial_update_before}\\
& \w_{t+1}^k =\left\{\begin{array}{ll}
\v_{t+1}^k           & \text{ if } t+1 \notin \IM_E, \\
\text{samples} \ \SM_{t+1} \text{ and average }  \{ \v_{t+1}^k\}_{k \in \SM_{t+1}}  & \text{ if } t+1  \in \IM_E.
\label{eq:partial_update_after}
\end{array}\right. 
\end{align}


\paragraph{Sources of randomness.}
In our analysis, there are two sources of randomness. One results from the stochastic gradients and the other is from the random sampling of devices. 
All the analysis in Appendix~\ref{appen:full} only involve the former. To distinguish them, we use the notation $\EB_{\SM_t}(\cdot)$, when we take expectation to erase the latter type of randomness. 


\subsection{Key Lemmas}
\paragraph{Two schemes.}
For full device participation, we always have $\aw_{t+1} = \av_{t+1}$. This is true when $t+1 \notin \IM_E$ for partial device participation. When $t{+}1 \in \IM_E$, we hope this relation establish in the sense of expectation. To that end, we require the sampling and averaging scheme to be unbiased in the sense that
\[  \EB_{\SM_{t+1}}  \aw_{t+1} = \av_{t+1}.  \]

We find two sampling and averaging schemes satisfying the requirement and provide convergence guarantees.
\begin{enumerate}[(I)]
	\item The server establishes $\SM_{t+1}$ by i.i.d. \textbf{with replacement} sampling an index $k \in \{1,\cdots,N\}$ with probabilities $p_1,\cdots,p_N$ for $K$ times. Hence $\SM_{t+1}$ is a multiset which allows a element to occur more than once. Then the server averages the parameters by $\w_{t+1}^k  = \frac{1}{K} \sum_{k \in \SM_{t+1}} \v_{t+1}^k$. This is first proposed in \citep{sahu2018convergence} but lacks theoretical analysis.
	\item The server samples $\SM_{t+1}$ uniformly in a \textbf{without replacement} fashion. Hence each element in $\SM_{t+1}$ only occurs once.Then server averages the parameters by $\w_{t+1}^k = \sum_{k \in \SM_{t+1}} p_{k} \frac{N}{K} \v_{t+1}^{k}$. Note that when the $p_k$'s are not all the same, one cannot ensure $\sum_{k \in \SM_{t+1}} p_{k} \frac{N}{K} = 1$.
\end{enumerate}

\paragraph{Unbiasedness and bounded variance.}
Lemma~\ref{lem:conv_v_w_e} shows the mentioned two sampling and averaging schemes are unbiased.
 In expectation, the next-round parameter (i.e., $\aw_{t+1}$) is equal to the weighted average of parameters in \textbf{all devices} after SGD updates (i.e., $\av_{t+1}$). However, the original scheme in \citep{mcmahan2016communication} (see Table~\ref{tab:conv}) does not enjoy this property. But it is very similar to Scheme II except the averaging scheme. Hence our analysis cannot cover the original scheme.
 
 Lemma~\ref{lem:conv_v_w} shows the expected difference between $\av_{t+1}$ and $\aw_{t+1}$ is bounded. $\ESt \left\| \av_{t+1} - \aw_{t+1} \right\|^2$ is actually the variance of $\aw_{t+1}$.
 

\begin{lem}[Unbiased sampling scheme]
	\label{lem:conv_v_w_e}
	If $t+1 \in \IM_E$, for Scheme I and Scheme II, we have
	\[
	\ESt (\aw_{t+1}) = \av_{t+1}.
	\]
\end{lem}


\begin{lem}[Bounding the variance of $\aw_t$]
	\label{lem:conv_v_w}
	For $t+1 \in \IM$, assume that $\eta_t$ is non-increasing and $\eta_{t} \le 2 \eta_{t+E}$ for all $t\geq 0$. We have the following results.
	\begin{enumerate}[(1)]
		\item For Scheme I, the expected difference between $\av_{t+1}$ and $\aw_{t+1}$ is bounded by
		\[
		\ESt \left\| \av_{t+1} - \aw_{t+1} \right\|^2 \leq \frac{4}{K} \eta_t^2 E^2 G^2.
		\]
		\item For Scheme II, assuming $p_1=p_2=\cdots=p_N=\frac{1}{N}$, the expected difference between $\av_{t+1}$ and $\aw_{t+1}$ is bounded by
		\[
		\ESt \left\| \av_{t+1} - \aw_{t+1} \right\|^2 \leq  \frac{N-K}{N-1} \frac{4}{K}\eta_t^2 E^2 G^2.
		\]
	\end{enumerate}
\end{lem}



\subsection{Completing the Proof of Theorem~\ref{thm:w_replace} and \ref{thm:wo_replace}}
\begin{proof}
Note that
\begin{align*}
\left\| \aw_{t+1} - \w^* \right\|^2  
&=    \left\| \aw_{t+1} - \av_{t+1} + \av_{t+1} - \w^* \right\|^2 \\
& = \underbrace{\left\| \aw_{t+1} - \av_{t+1} \right\|^2}_{A_1} +
\underbrace{\left\| \av_{t+1} - \w^* \right\|^2}_{A_2} +
\underbrace{2\langle \aw_{t+1} - \av_{t+1} , \av_{t+1} - \w^*  \rangle}_{A_3}.
\end{align*}	
When expectation is taken over $\SM_{t+1}$, the last term ($A_3$) vanishes due to the unbiasedness of $\aw_{t+1}$. 

If $t+1 \notin \IM_E$, $A_1$ vanishes since $\aw_{t+1} = \av_{t+1}$. We use Lemma~\ref{lem:conv_v_w} to bound $A_2$. Then it follows that
\[  \EB \left\| \aw_{t+1} - \w^* \right\|^2   \leq  (1-\eta_t \mu) \EB \left\|\aw_{t}-\w^{\star}\right\|^{2}  + \eta_t^2 B. \]

If $t+1 \in \IM_E$, we additionally use Lemma~\ref{lem:conv_v_w} to bound $A_1$. Then
\begin{align}
\label{eq:conv_final}
\EB \left\| \aw_{t+1} - \w^* \right\|^2  
& = \EB \left\| \aw_{t+1} - \av_{t+1} \right\|^2  + \EB \left\| \av_{t+1} - \w^* \right\|^2 \nonumber \\
& \leq  (1-\eta_t \mu) \EB \left\|\aw_{t}-\w^{\star}\right\|^{2}  + \eta_t^2 (B+ C),
\end{align}
where $C$ is the upper bound of $\frac{1}{\eta_t^2} \ESt \left\| \av_{t+1} - \aw_{t+1} \right\|^2$ ($C$ is defined in Theorem~\ref{thm:w_replace} and~\ref{thm:wo_replace}). 

The only difference between~\eqref{eq:conv_final} and~\eqref{eq:conv_full_final} is the additional $C$.
Thus we can use the same argument there to prove the theorems here.
Specifically, for a diminishing stepsize, $\eta_t = \frac{\beta}{t + \gamma}$ for some $\beta > \frac{1}{\mu}$ and $\gamma > 0$ such that $\eta_1 \le \min\{\frac{1}{\mu}, \frac{1}{4L}\}=\frac{1}{4L}$ and $\eta_{t} \le 2 \eta_{t+E}$, we can prove $\EB \left\| \aw_{t+1} - \w^* \right\|^2   \le \frac{v}{\gamma + t}$ where $v = \max\left\{ \frac{\beta^2 (B+C)}{\beta \mu -1}, (\gamma+1)\|\w_1 -\w^*\|^2\right\}$.

Then by the strong convexity of $F(\cdot)$,
\[  \EB [F(\aw_t)] - F^* \le \frac{L}{2} \Delta_t  \le \frac{L}{2} \frac{v}{\gamma + t}.\]
Specifically, if we choose $\beta = \frac{2}{\mu},\gamma = \max\{8 \frac{L}{\mu}, E\}-1$ and denote $\kappa = \frac{L}{\mu}$, then  $\eta_t = \frac{2}{\mu} \frac{1}{\gamma + t}$ and 
\[  \EB [F(\aw_t)] - F^* \le   \frac{\kappa}{\gamma + t} \left( \frac{2(B+C)}{\mu} +  \frac{ \mu (\gamma+1)}{2} \|\w_1 -\w^*\|^2 \right). \]
\end{proof}


\subsection{Deferred proofs of key lemmas}

\begin{proof}[Proof of Lemma~\ref{lem:conv_v_w_e}]
We first give a key observation which is useful to prove the followings. Let $\{x_i\}_{i=1}^N$ denote any fixed deterministic sequence. We sample a multiset $\SM_t$ (with size $K$) by the procedure where
for each sampling time, we sample $x_k$ with probability $q_k$ for each time. Pay attention that two samples are not necessarily independent. We only require each sampling distribution is identically. Let $\SM_t = \{i_1, \cdots, i_K\} \subset [N]$ (some $i_k$'s may have the same value). Then
\[  \EB_{\SM_t}  \sumk x_k = \EB_{\SM_t}  \sum_{k=1}^K x_{i_k} = K \EB_{\SM_t}  x_{i_1} = K \sum_{k=1}^Nq_k x_k. \]
For Scheme I, $q_k = p_k$ and for Scheme II, $q_k = \frac{1}{N}$. It is easy to prove this lemma when equipped with this observation.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:conv_v_w}]
	We separately prove the bounded variance for two schemes. Let $\SM_{t+1} = \{i_1, \cdots, i_K \} $ denote the multiset of chosen indexes.
	
	(1) For Scheme I, $\aw_{t+1} = \frac{1}{K} \sum_{l=1}^K \v_{t+1}^{i_l}$. Taking expectation over $\SM_{t+1}$, we have
	
	\begin{equation}
	\label{eq:v_s1}
	\ESt \left\| \aw_{t+1} - \av_{t+1} \right\|^2 
= \ESt \frac{1}{K^2} \sum_{l=1}^K \left\| \v_{t+1}^{i_l} - \av_{t+1} \right\|^2 
=  \frac{1}{K} \sum_{k=1}^N p_k \left\| \v_{t+1}^{k} - \av_{t+1} \right\|^2
	\end{equation}
	where the first equality follows from $\v_{t+1}^{i_l}$ are independent and unbiased.
	
	To bound~\eqref{eq:v_s1}, we use the same argument in Lemma~\ref{lem:conv_v_w}. Since $t+1 \in \IM_E$, we know that the time $t_0 = t - E +1 \in \IM_E$ is the communication time, which implies  $\{\w_{t_0}^k\}_{k=1}^N$ is identical. Then 
	\begin{align*}
	\myave \left\| \v_{t+1}^{k} - \av_{t+1} \right\|^2 
	&=  \myave \left\| (\v_{t+1}^{k} - \aw_{t_0}) - ( \av_{t+1} - \aw_{t_0} ) \right\|^2 \\
	&\leq \myave \left\|\v_{t+1}^{k} - \aw_{t_0} \right\|^2
	\end{align*}
	where the last inequality results from $\myave (\v_{t+1}^k - \aw_{t_0}) = \av_{t+1} - \aw_{t_0}$ and $\EB \| \vx-\EB \vx \|^2 \leq \EB \| \vx \|^2$. Similarly, we have
	\begin{align*}
	\ESt \left\| \aw_{t+1} - \av_{t+1} \right\|^2 
	& \leq \frac{1}{K}   \myave \EB \left\|\v_{t+1}^k - \aw_{t_0} \right\|^2 \\
	& \leq \frac{1}{K}   \myave \EB \left\|\v_{t+1}^k - \w_{t_0}^k \right\|^2 \\
	& \leq \frac{1}{K} \myave   E \sum_{i=t_0}^t \EB \left\| \eta_i \nabla F_k(\w_i^k, \xi_i^k) \right\|^2 \\
	& \leq  \frac{1}{K} E^2 \eta_{t_0}^2 G^2 \leq \frac{4}{K} \eta_t^2 E^2 G^2
	\end{align*}
	where in the last inequality we use the fact that $\eta_t$ is non-increasing and $\eta_{t_0} \leq 2 \eta_t$.
	
	(2) For Scheme II, when assuming $p_{1}=p_{2}=\cdots=p_{N}=\frac{1}{N}$, we again have $\aw_{t+1} = \frac{1}{K} \sum_{l=1}^K \v_{t+1}^{i_l}$.
	
	\begin{align*}
	\ESt& \left\| \aw_{t+1} - \av_{t+1} \right\|^2 = \ESt \left\| \frac{1}{K} \sum_{i \in S_{t+1}} \v_{t+1}^i - \av_{t+1} \right\|^2 = \frac{1}{K^2} \ESt \left\|  \sum_{i=1}^N \IB{i \in S_t} (\v_{t+1}^i - \av_{t+1}) \right\|^2\\
	& = \frac{1}{K^2} \left[\sum_{i \in [N]}
	\PB\left(i \in S_{t+1}\right) \left\|  \v_{t+1}^i - \av_{t+1} \right\|^2 +
	\sum_{i\ne j} \PB\left( i,j \in S_{t+1}\right) \langle  \v_{t+1}^i - \av_{t+1} , \v_{t+1}^j - \av_{t+1} \rangle 
	\right]\\
	& = \frac{1}{KN}  \sum_{i=1}^N   \left\|  \v_{t+1}^i - \av_{t+1} \right\|^2 
	+ \sum_{i\ne j} \frac{K-1}{KN(N-1)}  \langle  \v_{t+1}^i - \av_{t+1} , \v_{t+1}^j - \av_{t+1}\rangle  \\
	& = \frac{1}{K(N-1)}\left(1-\frac{K}{N}\right) \sum_{i=1}^N \left\| \v_{t+1}^i - \av_{t+1} \right\|^2
	\end{align*}
	where we use the following equalities: (1) $\PB\left(i \in S_{t+1}\right) = \frac{K}{N}$ and $ \PB\left( i,j \in S_{t+1}\right) = \frac{K(K-1)}{N(N-1)}$ for all $i \ne j$ and (2)  $\sum_{i \in [N]} \left\|  \v_{t+1}^i - \av_{t+1} \right\|^2 +
	\sum_{i\ne j}  \langle  \v_{t+1}^i - \av_{t+1} , \v_{t+1}^j - \av_{t+1}\rangle = 0$.
	
	Therefore,
	\begin{align*}
	\EB \left\| \aw_{t+1} - \av_{t+1} \right\|^2 
	& =  \frac{N}{K(N-1)}\left(1-\frac{K}{N}\right) \EB\left[ \frac{1}{N} \sum_{i=1}^N \left\| \v_{t+1}^i - \av_{t+1} \right\|^2 \right] \\
	& \leq \frac{N}{K(N-1)}\left(1-\frac{K}{N}\right) \EB\left[ \frac{1}{N} \sum_{i=1}^N \left\| \v_{t+1}^i - \aw_{t_0} \right\|^2 \right] \\
	& \leq \frac{N}{K(N-1)}\left(1-\frac{K}{N}\right) 4 \eta_t^2 E^2 G^2.
	\end{align*}
	where in the last inequality we use the same argument in (1).
\end{proof}



==> tex/details.tex <==
\section{Experimental Details}
\label{sec:appen:exp}
\subsection{Experimental Setting}
\paragraph{Model and loss.}
We examine our theoretical results on a multinomial logistic regression. Specifically, let $f(\w;x_i)$  denote the prediction model with the parameter $\w = (\W, \bb)$ and the form $f(\w;\x_i) = \text{softmax}(\W\x_i+\bb)$. The loss function is given by
\[F(\w) = \frac{1}{n}\sum_{i=1}^n \text{CrossEntropy}\left(f(\w;\x_i), \y_i \right) + \lambda \|\w\|_2^2.  \]
This is a convex optimization problem. The regularization parameter is set to $\lambda = 10^{-4}$.

\paragraph{Datasets.}
We evaluate our theoretical results on both real data and synthetic data. For real data, we choose MNIST dataset \citep{lecun1998gradient} because of its wide academic use. To impose statistical heterogeneity, we distribute the data among $N=100$ devices such that each device contains samples of only two digits. To explore the effect of data unbalance, we further vary the number of samples among devices. Specifically, for unbalanced cases, the number of samples among devices follows a power law, while for balanced cases, we force all devices to have the same amount of samples. 

Synthetic data allow us to manipulate heterogeneity more precisely. Here we follow the same setup as described in \citep{sahu2018convergence}. In particular, we generate synthetic samples $(\X_k, \Y_k)$ according to the model $ y = \argmax(\text{softmax}(\W_k x+\bb_k))$ with $x \in \RB^{60}, \W_k \in \RB^{10 \times 60}$ and $\bb_k \in \RB^{10}$, where $\X_k \in \RB^{n_k \times 60}$ and $\Y_k \in \RB^{n_k}$. We model each entry of $\W_k$ and $\bb_k$ as $\NM(\mu_k, 1)$ with $\mu_k \sim \NM(0, \alpha)$, and $(x_{k})_{j} \sim \NM(v_k, \frac{1}{j^{1.2}})$ with $v_k \sim \NM(B_k, 1)$ and $B_k \sim \NM(0, \beta)$. Here $\alpha$ and $\beta$ allow for more precise manipulation of data heterogeneity: $\alpha$ controls how much local models differ from each other and $\beta$ controls how much the local data at each device differs from that of other devices. There are $N=100$ devices in total. The number of samples $n_k$ in each device follows a power law, i.e., data are distributed in an unbalanced way. We denote by synthetic$(\alpha,\beta)$ the synthetic dataset with parameter $\alpha$ and $\beta$.

We summarize the information of federated datasets in Table~\ref{tab:data}.


\paragraph{Experiments.}
For all experiments, we initialize all runnings with $\w_0 = 0$. In each round, all selected devices run $E$ steps of SGD in parallel. We decay the learning rate at the end of each round by the following scheme $\eta_t = \frac{\eta_0}{1+t}$, where $\eta_0$ is chosen from the set $\{1, 0.1, 0.01\}$. We evaluate the averaged model after each global synchronization on the corresponding global objective. For fair comparison, we control all randomness in experiments so that the set of activated devices is the same across all different algorithms on one configuration.


\begin{table}
	\caption{Statistics of federated datasets}
	\label{tab:data}
	\centering
	\begin{tabular}{cccccc}
		\toprule
		Dataset & Details & $\#$ Devices $(N)$ & $\#$Training samples $(n)$ & \multicolumn{2}{c}{Samples/device}\\
		\cmidrule(r){5-6}
		&   &   &   &  mean     & std     \\
		\midrule
		\multirow{2}{*}{MNIST} 
		& balanced       & 100 & 54200 & 542 & 0\\
		& unbalanced & 100 & 62864 & 628  & 800 \\
		\midrule
		\multirow{2}{*}{Synthetic Data} 
		& $\alpha=0,\beta=0$ &100& 42522 & 425 & 1372 \\
		& $\alpha=1,\beta=1$ &100& 27348 & 273 & 421  \\
		\bottomrule
	\end{tabular}
\end{table}

\subsection{Theoretical verification}

\paragraph{The impact of $E$.}
From our theory, when the total steps $T$ is sufficiently large, the required number of communication rounds to achieve a certain precision is
\begin{equation*}
T_\epsilon/E \approx 
\frac{T_\epsilon}{E} 
\: \propto \:   \left(1+\frac{1}{K}\right)EG^2 + \frac{\myave ^2\sigma_k^2 + L \Gamma + \kappa G^2}{E} + G^2 ,
\end{equation*}
which is s a function of $E$ that first decreases and then increases. This implies that the optimal local step $E^*$ exists. What's more, the $T_\epsilon/E$ evaluated at $E^*$ is
\[ \mathcal{O}\left( G\sqrt{\myave ^2\sigma^2 +L\Gamma + \kappa G^2 }  \right), \] 
which implies that \texttt{FedAvg} needs more communication rounds to tackle with severer heterogeneity.

To validate these observations, we test \texttt{FedAvg} with Scheme I on our four datasets as listed in Table~\ref{tab:data}. In each round, we activate $K=30$ devices and set $\eta_0=0.1$ for all experiments in this part. For unbalanced MNIST, we use batch size $b=64$. The target loss value is $0.29$ and the minimum loss value found is $0.2591$. For balanced MNIST, we also use batch size $b=64$. The target loss value is $0.50$ and the minimum loss value found is $0.3429$. For two synthetic datasets, we choose $b=24$. The target loss value for synthetic(0,0) is $0.95$ and the minimum loss value is $0.7999$. Those for synthetic(1,1) are $1.15$ and $1.075$.

\paragraph{The impact of $K$.}
Our theory suggests that a larger $K$ may accelerate convergence since $T_\epsilon/E $ contains a term $\mathcal{O}\left( \frac{EG^2}{K}\right)$. We fix $E=5$ and $\eta_0=0.1$ for all experiments in this part. We set the batch size to 64 for two MNIST datasets and 24 for two synthetic datasets. We test Scheme I for illustration. Our results show that, no matter what value $K$ is, \texttt{FedAvg} converges. From Figure~\ref{fig:K}, all the curves in each subfigure overlap a lot. To show more clearly the differences between the curves, we zoom in the last few rounds in the upper left corner of the figure. It reveals that the curve of a large enough $K$ is slightly better. This result also shows that there is no need to sample as many devices as possible in convex federated optimization.

\begin{figure}[ht]
	\centering
	\subfloat[Balanced MNIST]{
		\includegraphics[width=0.4\textwidth] {fig/mnist_balanced_K.pdf}}
	\subfloat[Unbalanced MNIST]{
		\includegraphics[width=0.4\textwidth] {fig/mnist_unbalanced_K.pdf}}
	\\
	\subfloat[Synthetic(0, 0)]{
		\includegraphics[width=0.4\textwidth] {fig/alpha0_beta0_niid_K.pdf}}
	\subfloat[Synthetic(1, 1)]{
		\includegraphics[width=0.4\textwidth] {fig/alpha1_beta1_niid_K.pdf}}
	\caption{The impact of $K$ on four datasets. To show more clearly the differences between the curves, we zoom in the last few rounds in the upper left corner of the box.}
	\label{fig:K}
\end{figure}

\paragraph{Sampling and averaging schemes.}
We analyze the influence of sampling and averaging schemes. As stated in Section~\ref{subsec:conv_partial}, \textbf{Scheme I} iid samples (with replacement) $K$ indices with weights $p_k$ and simply averages the models, which is proposed by \citet{sahu2018convergence}. \textbf{Scheme II} uniformly samples (without replacement) $K$ devices and weightedly averages the models with scaling factor $N/K$. \textbf{Transformed Scheme II} scales each local objective and uses uniform sampling and simple averaging. We compare Scheme I, Scheme II and transformed Scheme II, as well as the original scheme~\citep{mcmahan2016communication} on four datasets. We carefully tuned the learning rate for the original scheme. In particular, we choose the best step size from the set $\{0.1, 0.5, 0.9, 1.1\}$. We did not fine tune the rest schemes and set $\eta_0 = 0.1$ by default. The hyperparameters are the same for all schemes: $E=20, K=10$ and $b=64$. The results are shown in Figure~\ref{fig:test_figure_c} and~\ref{fig:test_figure_d}.

Our theory renders Scheme I the guarantee of convergence in common federated setting. As expected,  Scheme I performs well and stably across most experiments. This also coincides with the findings of \citet{sahu2018convergence}. They noticed that Scheme I performs slightly better than another scheme: server first uniformly samples devices and then averages local models with weight $p_k/\sum_{l \in S_t}p_l$. However, our theoretical framework cannot apply to it, since for $t \in \IM$, $\EB_{S_t} \aw_t = \av_t$ does not hold in general.

Our theory \textbf{does not} guarantee \texttt{FedAvg} with Scheme II could converge when the training data are unbalanced distributed. Actually, if the number of training samples varies too much among devices, Scheme II may even diverge. To illustrate this point, we have shown the terrible performance on \texttt{mnist unbalanced} dataset in Figure~\ref{fig:test_figure_b}. In Figure~\ref{fig:more_scheme}, we show additional results of Scheme II on the two synthetic datasets, which are the most unbalanced. We choose $b=24, K=10, E=10$ and $\eta_0=0.1$ for these experiments. However, transformed Scheme II performs well except that it has a lower convergence rate than Scheme I.


\begin{figure}[ht]
	\centering
	\subfloat[Synthetic(0,0)]{
		\includegraphics[width=0.4\textwidth] {fig/synthetic0_0_scheme.pdf}}
	\subfloat[Synthetic(1,1)]{
		\includegraphics[width=0.4\textwidth] {fig/synthetic1_1_scheme.pdf}}
	\caption{The performance of four schemes on two synthetic datasets. The Scheme I performs stably and the best. The original performs the second. The curve of the Scheme II fluctuates and has no sign of convergence. Transformed Scheme II has a lower convergence rate than Scheme I.}
	\label{fig:more_scheme}
\end{figure}


==> tex/new_proof.tex <==

\section{New proof}

\subsection{Additional Notation}

Let $\w_t^k$ be the model parameter maintained in the $k$-th device at the $t$-th step. Let $\IM $ be the set of global synchronization steps, i.e., $\IM_E = \{nE \  | \ n=1,2,\cdots\}$. If $t+1 \in \IM_E$, i.e., the time step to communication, \texttt{FedAvg} randomly activates a subset of devices with the probability $p_k$. We denote by $\HM_t$ the multiset selected which is only well defined for $t \in \IM$. For convenience, we denote by $\SM_t = \HM_{N(t, E)}$ where $N(t, E) = \max\{n| n \le t, n \in \IM_E\}$. Then the update of \texttt{FedAvg} with partial devices active can be described as
\begin{align}
& \v_{t+1}^k = \w_t^k - \eta_t \nabla F_k(\w_t^k, \xi_t^k), 
\label{eq:partial_update_before}\\
& \w_{t+1}^k =\left\{\begin{array}{ll}
\v_{t+1}^k           & \text{ if } t+1 \notin \IM_E, \\
 \frac{1}{K}\sum_{k \in \SM_t}\v_{t+1}^k   & \text{ if } t+1  \in \IM_E.
 \label{eq:partial_update_after}
\end{array}\right. 
\end{align}
Here, an additional variable $\v_{t+1}^k$ is introduced to represent the immediate result of one step SGD update from $\w_t^k$. 

We define a virtual sequence $\overline{\v}_{t+1} = \frac{1}{K}\sum_{k \in \SM_t}\v_{t+1}^k$, the sample mean of updated parameters which are maintained in activated devices. Note that $\overline{\v}_{t+1}$ is inaccessible when $t+1 \in \IM_E$. When $t+1 \in \IM_E$, for all activated devices $k \in \HM_{t+1}$, $\w_{t+1}^k = \overline{\v}_{t+1}$ and hence $\overline{\w}_{t+1}=\overline{\v}_{t+1}$. 

In our analysis, there are two sources of randomness. One results from the stochastic gradients and the other is from the random sampling of devices. When we take expectation, we should distinguish them. To that end, we denote by $\EB_{\GM}(\cdot)$ the former type and $\EB_{\SM_t}(\cdot)$ the latter. 

Further, we define $\overline{\g}_t = \frac{1}{K}\sum_{k \in \SM_t} \nabla F_k(\w_t^k)$ and $\g_t = \frac{1}{K}\sum_{k \in \SM_t} \nabla F_k(\w_t^k, \xi_t^k)$. Then $\overline{\v}_{t+1} = \overline{\w}_t - \eta_t \g_t$ and $\EB_{\GM} \g_t = \overline{\g}_t$.


\subsection{Key Lemmas}
To convey our proof clearly, it would be necessary to prove certain useful lemmas. We defer the proof of these lemmas to latter section and focus on proving the main theorem.

\begin{lem}[Results of one step SGD]
\label{lem:partial_main_lem1} Assume Assumption~\ref{asm:smooth} and~\ref{asm:strong_cvx}. If $\eta_t\leq \frac{1}{4L}$, then conditioning on $\SM_t$, we have
\begin{align*}
\EB_{\GM} \left\|\av_{t+1}-\w^{\star}\right\|^{2} 
&\leq (1-\eta_t \mu) \EB_{\GM} \left\|\overline{\w}_{t}-\w^{\star}\right\|^{2} + 
\frac{2}{K} \sumk \EB_{\GM}  \| \overline{\w}_t - \w_t^k\|_2^2 +
 \eta_{t}^{2} \EB_{\GM} \left\|\mathbf{g}_{t}-\overline{\mathbf{g}}_{t}\right\|^{2}.
\\
& \quad
+ \frac{2\eta_t}{K} \sumk \left( F^* -F_k^* \right) 
+ \frac{2\eta_t}{K}\sumk \left(F_k(\w^*) - F^*\right)
\end{align*}
\end{lem}


\begin{lem}[Bounding the variance]
Assume Assumption~\ref{asm:sgd_var} holds and condition on $\SM_t$. It follows that
	\label{lem:partial_var}
	\[
	\EB_{\GM} \left\|\mathbf{g}_{t}-\overline{\mathbf{g}}_{t}\right\|^{2} 
	\leq \frac{\sumk \sigma_k^2}{K^2}.
	\]
\end{lem}


\begin{lem}[Bounding the divergence of $\{\w_t^k\}$]
	\label{lem:partial_diversity}
	Assume Assumption~\ref{asm:sgd_norm}, that $\eta_t$ is non-increasing and $\eta_{t+E} \leq 2 \eta_t$ for all $t\geq 0$. Then conditioning on $\SM_t$, we have
	\[
	\EB_{\GM} 
	\left[\frac{1}{K} \sumk \left\|\overline{\w}_{t}-\w_{k}^{t}\right\|^{2} \right]
	\: \leq \: 4 \eta_t^2 (E-1)^2 G^2.
	\]
\end{lem}


\begin{lem}
\label{lem:partial_main_lem2}
If $\eta_t\leq \frac{1}{4L}$,  we have
\begin{equation*}
\EB \left\|\av_{t+1}-\w^{\star}\right\|^{2} 
\leq (1-\eta_t \mu) \EB \left\|\overline{\w}_{t}-\w^{\star}\right\|^{2} 
+ \eta_t^2 B
\end{equation*}
where the expectation is taken for all randomness and 
\[ B =  8L\myave \left( F^* -F_k^* \right) + \frac{\myave \sigma_k^2}{K} + 8(E-1)^2 G^2.\]
\end{lem}

\begin{proof}[Proof of ]
No matter $t+1 \in \IM_E$ or $t+1 \notin \IM_E$, we always have $\aw_{t+1}= \av_{t+1}$. Let $\Delta_t=\EB \left\|\aw_{t+1}-\w^{\star}\right\|^{2}$. For a diminishing stepsize, $\eta_t = \frac{\beta}{t + \gamma}$ for some $\beta > \frac{1}{\mu}$ and $\gamma > 0$ such that $\eta_1 \le \min\{\frac{1}{\mu}, \frac{1}{4L}\}$. We prove $\Delta_t \le \frac{v}{\gamma + t}$ where $v = \max\left\{ \frac{\beta^2 B}{\beta \mu -1}, (\gamma+1)\Delta_1 \right\}$.

We prove it by induction. Firstly, the definition of $v$ ensures that it holds for $t = 1$. Assume the conclusion holds for some $t$, it follows that
\begin{align*}
\Delta_{t+1} 
&\le (1-\eta_t\mu )\Delta_t + \eta_t^2 B \\
&=\left(1- \frac{\beta\mu}{t + \gamma}\right)\frac{v}{t + \gamma} + \frac{\beta^2B}{(t + \gamma)^2}\\
&=\frac{t + \gamma -1}{(t + \gamma)^2} v  + \left[ \frac{\beta^2B}{(t + \gamma)^2} - \frac{\beta\mu-1}{(t+\gamma)^2}v \right] \\
& \le \frac{v}{t + \gamma +1}.
\end{align*}

Then by the strong convexity of $F(\cdot)$,
\[  F(\aw_t) - F^* \le \frac{L}{2} \Delta_t  \le \frac{L}{2} \frac{v}{\gamma + t}.\]
\end{proof}



\subsection{Deferred proofs of key lemmas}
\begin{proof}[Proof of Lemma~\ref{lem:partial_main_lem1}.]
	Notice that $\av_{t+1} = \aw_t - \eta_t \vg_t$, then
	\begin{align}
	\label{eq:partial_main}
	\left\|\overline{\v}_{t+1}-\w^{\star}\right\|^{2} \nonumber 
	&=\left\|\overline{\w}_{t}-\eta_{t} \mathbf{g}_{t}-\w^{\star}-\eta_{t} \overline{\mathbf{g}}_{t}+\eta_{t} \overline{\mathbf{g}}_{t}\right\|^{2} \nonumber \\ 
	&=\underbrace{\left\|\overline{\w}_{t}-\w^{\star}-\eta_{t} \overline{\mathbf{g}}_{t}\right\|^{2}}_{A_1}+
	\underbrace{2\eta_{t}\left\langle\overline{\w}_{t}-\w^{\star}-\eta_{t} \overline{\mathbf{g}}_{t}, \overline{\mathbf{g}}_{t}-\mathbf{g}_{t}\right\rangle}_{A_2} +
	\eta_{t}^{2}\left\|\mathbf{g}_{t}-\overline{\mathbf{g}}_{t}\right\|^{2}
	\end{align}
	Note that $\EB_{\GM} A_2 = 0$. We next focus on bounding $A_1$. Again we split $A_1$ into three terms:
	\begin{equation}
	\label{eq:partial_proof_main_term}
	\left\|\overline{\w}_{t}-\w^{\star}-\eta_{t} \overline{\mathbf{g}}_{t}\right\|^{2} =\left\|\overline{\w}_{t}-\w^{\star}\right\|^{2}
	\underbrace{-2 \eta_{t}\left\langle\overline{\w}_{t}-\w^{\star}, \overline{\mathbf{g}}_{t}\right\rangle}_{B_1}
	+  \underbrace{\eta_{t}^{2}\left\|\overline{\mathbf{g}}_{t}\right\|^{2}}_{B_2}
	\end{equation}
	
	From the the $L$-smoothness of $F_k(\cdot)$, it follows that
	\begin{equation}
	\label{eq:partial_proof_L}
	  \left\|\nabla F_k\left(\w_{t}^{k}\right)\right\|^{2} \leq 2 L\left(F_k\left(\w_{t}^{k}\right)-F_k^{\star}\right).
	\end{equation}
	By the convexity of $\left\| \cdot \right \|^2$ and~\eqref{eq:partial_proof_L}, we have
	\[
	B_2 = \eta_{t}^{2}\left\|\overline{\mathbf{g}}_{t}\right\|^{2} 
	\leq \frac{\eta_{t}^{2}}{K}\sumk\left\|\nabla F_k\left(\w_{t}^{k}\right)\right\|^{2}
	\leq \frac{2L\eta_t^2}{K} \sumk \left( F_k(\w_t^k) - F_k^*\right).
	\]
	Note that 
	\begin{align}
	\label{eq:partial_B1}
	  B_1 
	  &= -2 \eta_{t}\left\langle\overline{\w}_{t}-\w^{\star}, \overline{\mathbf{g}}_{t}\right\rangle 
	  = -\frac{2\eta_t}{K} \sumk \left\langle\overline{\w}_{t}-\w^{\star}, \nabla F_k(\w_t^k)\right\rangle \nonumber \\
	  &=-\frac{2\eta_t}{K} \sumk \left\langle\overline{\w}_{t}-\w_t^k, \nabla F_k(\w_t^k)\right\rangle
	  -\frac{2\eta_t}{K} \sumk \left\langle\w_t^k-\w^{\star}, \nabla F_k(\w_t^k)\right\rangle.
	\end{align}
	By Cauchy-Schwarz inequality and AM-GM inequality, we have
	\begin{equation}
	\label{eq:partial_B11}
	-2 \left\langle\overline{\w}_{t}-\w_t^{k}, \nabla F_k \left(\w_{t}^{k}\right)\right\rangle \leq \frac{1}{\eta_t} \left\|\overline{\w}_{t}-\w_{t}^{k}\right\|^{2}
	+ \eta_t \left\|\nabla F_k\left(\w_{t}^{k}\right)\right\|^{2}.	
	\end{equation}
	By the $\mu$-strong convexity of $F_k(\cdot)$, we have
	\begin{equation}
	\label{eq:partial_B12}
	-\left\langle\w_{t}^{k}-\w^{\star}, \nabla F_k\left(\w_{t}^{k}\right)\right\rangle \leq -\left(F_k\left(\w_{t}^{k}\right)-F_k(\w^*)\right)-\frac{\mu}{2}\left\|\w_{t}^{k}-\w^{\star}\right\|^{2}.
	\end{equation}
	By combining ~\eqref{eq:partial_proof_main_term},~\eqref{eq:partial_B1},~\eqref{eq:partial_B11} and~\eqref{eq:partial_B12}, it follows that
	\begin{align*}
	 A_1 
	 =  \left\|\overline{\w}_{t}-\w^{\star}-\eta_{t} \overline{\mathbf{g}}_{t}\right\|^{2} 
	 &\leq \left\|\overline{\w}_{t}-\w^{\star}\right\|^{2} 
	 + \frac{2L\eta_t^2}{K} \sumk \left( F_k(\w_t^k) - F_k^*\right) \\
	 & \quad + \frac{\eta_t }{K}\sumk \left(\frac{1}{\eta_t} \left\|\overline{\w}_{t}-\w_{k}^{t}\right\|^{2}+\eta_t \left\|\nabla F_k\left(\w_{t}^{k}\right)\right\|^{2}\right)  \\ 
	&  \quad - \frac{2\eta_t}{K} \sumk \left( \left(F_k\left(\w_{t}^{k}\right)-F_k(\w^*)\right) + \frac{\mu}{2}\left\|\w_{t}^{k}-\w^{\star}\right\|^{2} \right) \\
	& = (1-\mu\eta_t)\left\|\overline{\w}_{t}-\w^{\star}\right\|^{2} 
	+ \frac{1}{K} \sumk \left\|\overline{\w}_{t}-\w_{k}^{t}\right\|^{2} \\
	& \quad + \underbrace{	\frac{4L\eta_t^2}{K} \sumk \left( F_k(\w_t^k) - F_k^*\right) 
	 - \frac{2\eta_t}{K} \sumk  \left(F_k\left(\w_{t}^{k}\right)-F_k(\w^*)\right)}_{C}
	\end{align*}
	where we use~\eqref{eq:partial_proof_L} again.
	
	We next aim to bound $C$. We define $\gamma_t = 2\eta_t(1-2L\eta_t)$. Since $\eta_t \leq \frac{1}{4L}$, $\eta_t \le \gamma_t \leq 2\eta_t$. Then we split $C$ into three terms:
	\begin{align*}
	 C &= - \frac{2\eta_t(1-2L\eta_t)}{K} \sumk \left( F_k(\w_t^k) - F_k^* \right) 
	 + \frac{2\eta_t}{K}\sumk \left(F_k(\w^*) - F_k^*\right) \\
	 &=-\frac{\gamma_t}{K}\sumk \left( F_k(\w_t^k) - F^* \right)  
	 -\frac{\gamma_t}{K}\sumk \left( F^*-F_k^*\right)  
	+ \frac{2\eta_t}{K}\sumk \left(F_k(\w^*) - F_k^*\right) \\
	 &=-\underbrace{\frac{\gamma_t}{K}\sumk \left( F_k(\w_t^k) - F^* \right)}_{D}
	 +\frac{4L\eta_t^2}{K}\sumk \left( F^*-F_k^*\right)  
	 + \frac{2\eta_t}{K}\sumk \left(F_k(\w^*) - F^*\right)
	\end{align*}
	To bound $D$, we have
	\begin{align*}
 \frac{1}{K} \sumk \left( F_k(\w_t^k) - F^*  \right)
	 &=\frac{1}{K} \sumk \left( F_k(\w_t^k) - F_k(\overline{\w}_t)  \right) 
	 + \frac{1}{K} \sumk \left( F_k(\overline{\w}_t) - F^*  \right)\\
	 & \ge \frac{1}{K} \sumk\left\langle \nabla F_k(\overline{\w}_t), \overline{\w}_t^k - \overline{\w}_t \right\rangle
	 + \frac{1}{K} \sumk \left( F_k(\overline{\w}) - F^*  \right)\\
	 & \ge - \frac{1}{2K}\sumk \left[ \eta_t\left\|  \nabla F_k(\overline{\w}_t) \right\|^2 + \frac{1}{\eta_t}\left\|\w_t^k -\overline{\w}_t\right\|^2 \right]
	 + \frac{1}{K} \sumk \left( F_k(\overline{\w}_t) - F^*  \right)\\
	 & \ge - \frac{1}{K}\sumk \left[ \eta_tL \left(F_k(\overline{\w}_t) -F_k^*   \right)
	 + \frac{1}{2\eta_t}\left\|\w_t^k -\overline{\w}_t\right\|^2 \right]
	 + \frac{1}{K} \sumk \left( F_k(\overline{\w}_t) - F^*  \right)
	\end{align*}
	where the first inequality results from the convexity of $F_k(\cdot)$, the second inequality from AM-GM inequality and the third inequality from~\eqref{eq:partial_proof_L}.
	
	Therefore 
	\begin{align*}
	  C 
	  &= \frac{\gamma_t}{K}\sumk \left[ \eta_tL \left(F_k(\overline{\w}_t) -F_k^*   \right)
	 + \frac{1}{2\eta_t}\left\|\w_t^k -\overline{\w}_t\right\|^2 \right]
	 - \frac{\gamma_t}{K} \sumk \left( F_k(\overline{\w}_t) - F^*  \right) \\
	 & \quad +\frac{4L\eta_t^2}{K}\sumk \left( F^*-F_k^*\right)  
	 + \frac{2\eta_t}{K}\sumk \left(F_k(\w^*) - F^*\right)\\
	 &= \frac{\gamma_t}{K}(\eta_t L -1 ) \sumk \left(F_k(\aw_t) -F_k^* \right)
	 + \frac{4L\eta_t^2 + \gamma_t}{K} \sumk \left( F^* - F_k^*\right) \\
	 & \quad + \frac{\gamma_t}{2\eta_t K} \sumk \left\|\w_t^k -\overline{\w}_t\right\|^2 
	 + \frac{2\eta_t}{K} \sumk \sumk \left(F_k(\w^*) - F^*\right)\\
	 &\le \frac{4L\eta_t^2}{K} \sumk \left( F^* - F_k^*\right)
	 + \frac{1}{K} \sumk \left\|\w_t^k -\overline{\w}_t\right\|^2 
	 + \frac{2\eta_t}{K} \sumk \left(F_k(\w^*) - F^*\right)
	\end{align*}
	where in the last inequality, we use the following facts: (1) $\eta_t L -1 \le - \frac{3}{4} \le 0$ and  $F_k(\aw_t) -F_k^*\ge 0$ and (2) $\frac{\gamma_t}{2\eta_t} \le 1$.
	
	Recalling the expression of $A_1$ and plugging $C$ into it, we have
	\begin{align}
	\label{eq:partial_proof_A1}
	  A_1 
	  &= \left\|\overline{\w}_{t}-\w^{\star}-\eta_{t} \overline{\mathbf{g}}_{t}\right\|^{2} \nonumber\\
      &\le (1-\mu\eta_t)\left\|\overline{\w}_{t}-\w^{\star}\right\|^{2} 
	  + \frac{2}{K} \sumk \left\|\overline{\w}_{t}-\w_{k}^{t}\right\|^{2} \nonumber \\
	  & \quad + \frac{1}{K} \sumk \left\|\w_t^k -\overline{\w}_t\right\|^2 
	 + \frac{2\eta_t}{K} \sumk \left(F_k(\w^*) - F^*\right)
	\end{align}
	Using~\eqref{eq:partial_proof_A1} and taking expectation on both sides of~\eqref{eq:partial_main}, we erase the randomness from stochastic gradients, we complete the proof.
\end{proof}



\begin{proof}[Proof of Lemma~\ref{lem:partial_var}]
    From Assumption~\ref{asm:sgd_var}, the variance of the stochastic gradients in device $k$ is bounded by $\sigma_k^2$, then
	\begin{align*}
	\EB_{\GM} \left\|\mathbf{g}_{t}-\overline{\mathbf{g}}_{t}\right\|^{2}  
	& = \EB \left\|\frac{1}{K} \sumk (\nabla F_k(\w_t^k,\xi_t^k) - \nabla F_k(\w_t^k))  \right\|^{2} \\
	&= \sumk \frac{1}{K^2} 
	\EB \left\|  \nabla F_k(\w_t^k,\xi_t^k) - \nabla F_k(\w_t^k)  \right\|^{2} \\
	& \leq \frac{1}{K^2} \sumk \sigma_k^2.
	\end{align*}
\end{proof}



\begin{proof}[Proof of Lemma~\ref{lem:partial_diversity}]
    Since \texttt{FedAvg} requires a communication each $E$ steps. Therefore, for any $t \ge 0$, there exists a $t_0 \leq t$, such that $t-t_0 \leq E-1$ and $\w_{t_0}^k=\aw_{t_0}$ for all $k=1,2,\cdots,N$. Also, we use the fact that $\eta_t$ is non-increasing and $\eta_{t_0} \leq 2 \eta_t$ for all $t-t_0 \leq E-1$, then
	\begin{align*}
	 \EB_{\GM} \sumk \frac{1}{K} \left\|\overline{\w}_{t}-\w_{k}^{t}\right\|^{2} 
	 &= \EB_{\GM} \frac{1}{K} \sumk \left\|  (\w_{k}^{t} - \aw_{t_0})  - (\overline{\w}_{t} - \aw_{t_0})   \right\|^{2} \\
	&\leq\EB_{\GM}  \sumk \frac{1}{K} \left\|  \w_{k}^{t} - \aw_{t_0}  \right\|^{2} \\
	& \leq \sumk \frac{1}{K} \EB_{\GM} \sum_{t = t_0}^{t-1}(E-1) \eta_t^2 \left\|  \nabla F_k(\w_k^{t},\xi_k^t)     \right\|^2 \\
	& \leq \sumk \frac{1}{K}\sum_{t=t_0} ^{t-1} (E-1) \eta_{t_0}^2 G^2 \\
	& \leq \sumk \frac{1}{K}  \eta_{t_0}^2 (E-1)^2 G^2 \\
	& \leq 4 \eta_t^2 (E-1)^2 G^2.
	\end{align*}
\end{proof}


\begin{proof}[Proof of Lemma~\ref{lem:partial_main_lem2}]
We first give a key observation which is useful to prove the followings. Let $\{x_i\}_{i=1}^N$ denote any fixed deterministic sequence. We sample a multiset $\SM_t$ (with size $K$) in an i.i.d. fashion with some probability $p_k$. Let $\SM_t = \{Y_1, \cdots, Y_K\} \subset [N]$ (some $Y_k$'s may have the same value but they are sampled independently). Then
\[  \EB_{\SM_t}  \sumk x_k = \EB_{\SM_t}  \sum_{k=1}^K x_{Y_k} = K \EB_{\SM_t}  x_{Y_1} = K\myave x_k. \]
Equipped with this observation, from Lemma~\ref{lem:conv_variance}, we have
\[ \EB \left\|\mathbf{g}_{t}-\overline{\mathbf{g}}_{t}\right\|^{2} 
= \EB_{\SM_t} \EB_{\GM} \left\|\mathbf{g}_{t}-\overline{\mathbf{g}}_{t}\right\|^{2}   
\le \EB_{\SM_t} \frac{1}{K^2} \sumk \sigma_k^2 = \frac{\myave \sigma_k^2}{K}. \]
From Lemma~\ref{lem:partial_diversity}, we have
\[ \EB \sumk \frac{1}{K} \left\|\overline{\w}_{t}-\w_{k}^{t}\right\|^{2}  
= \EB_{\SM_t} \EB_{\GM} \sumk \frac{1}{K} \left\|\overline{\w}_{t}-\w_{k}^{t}\right\|^{2}
\le 4 \eta_t^2 (E-1)^2 G^2.   \]
Similarly, it follows that $\EB_{\SM_t} \frac{1}{K}\sumk \left(F_k(\w^*) - F^*\right) = \myave \left(F_k(\w^*) - F^*\right) = 0$ and
\[  \EB_{\SM_t} \frac{1}{K} \sumk \left( F^* - F_k^* \right) =\myave \left(F^* -F_k^* \right) = \Gamma. \]

Combine this results and recall Lemma~\ref{lem:partial_main_lem1}. Then we finish the proof.
\end{proof}
